Certified Monotonic Neural Networks

Learning monotonic models with respect to a subset of the inputs is a desirable feature to effectively address the fairness, interpretability, and generalization issues in practice. Existing methods for learning monotonic neural networks either require specifically designed model structures to ensure monotonicity, which can be too restrictive/complicated, or enforce monotonicity by adjusting the learning process, which cannot provably guarantee the learned model is monotonic on selected features. In this work, we propose to certify the monotonicity of the general piece-wise linear neural networks by solving a mixed integer linear programming problem.This provides a new general approach for learning monotonic neural networks with arbitrary model structures. Our method allows us to train neural networks with heuristic monotonicity regularizations, and we can gradually increase the regularization magnitude until the learned network is certified monotonic. Compared to prior works, our approach does not require human-designed constraints on the weight space and also yields more accurate approximation. Empirical studies on various datasets demonstrate the efficiency of our approach over the state-of-the-art methods, such as Deep Lattice Networks.

==> tex/related.tex <==
\paragraph{Monotonic Models:}Monotonic models have been developed for decades, and isotonic regression is one of the most classical methods~\citep{dykstra2012advances}. Beyond isotonic regression, people also proposed methods to incorporate monotonic constraints to support vector machines~\citep{doumpos2009monotonic, chen2014credit}, decision trees~\citep{xgboost, pei2018partially, sharma2020testing}, neural networks~\citep{archer1993application, minin2010comparison, daniels2010monotone, you2017deep}, etc.. \citep{nguyen2019mononet}~incorporates monotonic constraints in training to obtain interpretable models.

\paragraph{Monotonic Neural Networks:}Learning monotonic neural network by setting all weights to positive can be traced back to 1993~\citep{archer1993application}. This method is simple, but the flexibility of the network is limited~\citep{daniels2010monotone}. \citep{sill1998monotonic} designed a fully monotonic network with monotonic linear layer and max-min pooling. Based on the results of~\citep{sill1998monotonic}, \citep{daniels2010monotone} proposed to use min-max pooling to build partially monotonic networks. The authors proved that the proposed architecture can universally approximate any partial monotone function. Recent advances in monotonic network leveraged a special structure, ensemble of lattices, and carefully constrained the parameters in the network to ensure monotonicity~\citep{fard2016fast, you2017deep}. Different from the previous works, our method does not require complicated network architecture or human-designed constraints on parameters.

\paragraph{Neural Network Verification:}The goal of neural network verification is to verify the properties of a neural network mathematically (e.g., will the output of the network always larger than 1 given that the input is bounded in $[0,1]$?)~\citep{bunel2018unified}. These kind of problems can often be transformed into solving an optimization problem. Most of the works in this field focus on evaluating the robustness of a network against adversarial attack~\citep{tjeng2017evaluating, raghunathan2018certified, zhang2019recurjac}. Neural network with piecewise linear activation function can be formulated as mixed integer linear programming~\citep{fischetti2017deep}, and this formulation enables verification via MILP solvers~\citep{bunel2018unified, tjeng2017evaluating}. Algorithms using MILP formulation have the ability to give exact solution of a verification problem, at the cost of computational time. To improve the speed of verification, we propose to do our monotonic verification in a layer-wise style. Another way for high-speed verification is performing relaxation on the original optimization problem~\citep{raghunathan2018certified, zhang2019recurjac}, but they are only accurate in a small region. Instead, our monotonic verification requires accuracy on the whole input space.
